Eclectic Rule Extraction for Explainability of Deep Neural Network based Intrusion Detection Systems

This paper addresses trust issues created from the ubiquity of black box algorithms and surrogate explainers in Explainable Intrusion Detection Systems (X-IDS). While Explainable Artificial Intelligence (XAI) aims to enhance transparency, black box surrogate explainers, such as Local Interpretable Model-Agnostic Explanation (LIME) and SHapley Additive exPlanation (SHAP), are difficult to trust. The black box nature of these surrogate explainers makes the process behind explanation generation opaque and difficult to understand. To avoid this problem, one can use transparent white box algorithms such as Rule Extraction (RE). There are three types of RE algorithms: pedagogical, decompositional, and eclectic. Pedagogical methods offer fast but untrustworthy white-box explanations, while decompositional RE provides trustworthy explanations with poor scalability. This work explores eclectic rule extraction, which strikes a balance between scalability and trustworthiness. By combining techniques from pedagogical and decompositional approaches, eclectic rule extraction leverages the advantages of both, while mitigating some of their drawbacks. The proposed Hybrid X-IDS architecture features eclectic RE as a white box surrogate explainer for black box Deep Neural Networks (DNN). The presented eclectic RE algorithm extracts human-readable rules from hidden layers, facilitating explainable and trustworthy rulesets. Evaluations on UNSW-NB15 and CIC-IDS-2017 datasets demonstrate the algorithm's ability to generate rulesets with 99.9% accuracy, mimicking DNN outputs. The contributions of this work include the hybrid X-IDS architecture, the eclectic rule extraction algorithm applicable to intrusion detection datasets, and a thorough analysis of performance and explainability, demonstrating the trade-offs involved in rule extraction speed and accuracy.

==> Tables/layers_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrrrrrl}
\hhline{==========}
\multicolumn{1}{c}{\textbf{Layers}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Prediction \\ Accuracy\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}True \\ Accuracy\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Total\\ Rules\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ Terms\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Longest\\ Rule\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Extraction\\ Time\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Testing\\ Time\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Testing\\ Std.\end{tabular}}} \\ \hline
\multicolumn{1}{l|}{Unbounded}      & \multicolumn{1}{r|}{0.999}                                                                  & \multicolumn{1}{r|}{0.931}                                                            & \multicolumn{1}{r|}{1686}                                                          & \multicolumn{1}{r|}{14.2}                                                         & \multicolumn{1}{r|}{27}                                                             & \multicolumn{1}{r|}{9504}                                                              & \multicolumn{1}{r|}{6962}                                                           & \multicolumn{1}{r}{1511}                                                            \\
\multicolumn{1}{l|}{20}             & \multicolumn{1}{r|}{0.999}                                                                  & \multicolumn{1}{r|}{0.931}                                                            & \multicolumn{1}{r|}{1675}                                                          & \multicolumn{1}{r|}{13.2}                                                         & \multicolumn{1}{r|}{20}                                                             & \multicolumn{1}{r|}{4401}                                                              & \multicolumn{1}{r|}{4659}                                                           & 1409                                                                                \\
\multicolumn{1}{l|}{10}             & \multicolumn{1}{r|}{0.996}                                                                  & \multicolumn{1}{r|}{0.929}                                                            & \multicolumn{1}{r|}{601}                                                           & \multicolumn{1}{r|}{9.1}                                                          & \multicolumn{1}{r|}{10}                                                             & \multicolumn{1}{r|}{2060}                                                              & \multicolumn{1}{r|}{1242}                                                           & 301                                                                                 \\
\multicolumn{1}{l|}{5}              & \multicolumn{1}{r|}{0.969}                                                                  & \multicolumn{1}{r|}{0.909}                                                            & \multicolumn{1}{r|}{57}                                                            & \multicolumn{1}{r|}{4.9}                                                          & \multicolumn{1}{r|}{5}                                                              & \multicolumn{1}{r|}{760}                                                               & \multicolumn{1}{r|}{113}                                                            & 30            
\hhline{=========}
\end{tabular}%
}
\end{table}

==> Tables/test_table.tex <==
\begin{table}[]
\begin{tabular}{lllll}
                          & 250                                                                                  & 300                                                                                  & 1000                                                                                 & 2000 \\ \cline{2-4}
\multicolumn{1}{l|}{0.01} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0/.05/.38\\ (0/.80/.42)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0/.05/.38\\ (0/.80/.42)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0/.17/.44\\ (0/.24/.50)\end{tabular}} &      \\ \cline{2-4}
\multicolumn{1}{l|}{0.02} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0/.05/.41\\ (0/.11/.50)\end{tabular}} & \multicolumn{1}{l|}{}                                                                & \multicolumn{1}{l|}{}                                                                &      \\ \cline{2-4}
                          &                                                                                      &                                                                                      &                                                                                      &     
\end{tabular}
\end{table}

==> intro_v1.tex <==
\section{Introduction}
Black-box Artificial Intelligence (AI) has become a popular solution for many domains. Intrusion Detection Systems, in particular, have seen an increase in black-box AI use due to their ability to discover \textit{zero-day} attacks \todo{i dont think this is the right claim to make in the opening, motivate using explainability}. A major issue that is arising with the use of these black-box systems is their low interpretability. This issue can cause a lack of trust in models, especially IDS. Explainable Intrusion Detection Systems (X-IDS) are a potential solution that can help increase trust. However, many current approaches in X-IDS utilize black-box explainers. 
%Achieving verifiable explainability in black-box Machine Learning (ML) is difficult. 
Black box explainers may not provide a reasonable degree of trust due to their black box nature. Explainability in practical Machine Learning (ML) can be hard to establish because many approaches map a set of inputs onto an output with little explanation of how the mapping occurs. Black-box explainability tasks may involve exploring the results of complex classification algorithms and generating valid explanations with post hoc methods. In eXplainable AI (XAI), results are verifiable, and each set of results can be used to improve future iterations of the model \cite{samek2017explainable, gunning2019darpa}. The desire for explainability in IDS stems from the fact that IDS are often associated with systems that utilize complex black-box architectures. These black-box systems are used to make decisions that protect user data, and it is vital that any IDS that is in a decision pipeline be trustworthy.
%It is vital that users who are making these decisions are able to trust the IDS that they are basing their actions on. 
%Explainability entails trust, and many users want to be able to trust an IDS system to make valid decisions \hl{[CITATION NEEDED]}.

Despite the application of Artificial Neural Networks (ANNs) in IDS, automated intrusion detection still requires human analysis \cite{axelsson2000intrusion}. Once an IDS detects an intrusion, it is necessary for analysts to determine that the predictions of the IDS are valid. There are many penalties for incorrectly flagged interactions, within large systems \cite{pietraszek2004using}. In \cite{morcos2022surrogate, joo2003neural}, the authors present the need for explainability in IDS systems with respect to the human-aspect, they also highlight the fact that high false positive and false negative rates in IDS may have severe consequences for organizations. For example, false positive results may lead to false accusations, and false negative results may allow an unauthorized entry \cite{ho2012statistical}. Specifically, trust should be addressed in all safety-critical systems to some degree \cite{dobbe2022system}. When responding to a potential intrusion, system administrators and security analysts will want to know the machine learning algorithms used within their IDS are trustworthy. Many intrusion detection systems utilize ANNs to generate highly accurate predictions. ANNs are inherently black box models \cite{szegedy2013intriguing}. When observing black box models, only the input and output are visible; therefore, explainability is more difficult in these scenarios. This raises the question: if only the input and output of an IDS are observed, how can the model's reliability be determined?

\textcolor{red}{A method that is ubiquitous for explaining ANN IDSs is to use black-box surrogate explainers.} Examples of surrogate explainers commonly used to explain the black box models are LIME \cite{Ribeiro2016}, SHAP \cite{Lundberg2017}, and LRP \cite{simonyan2013deep}. These explainers are black boxes themselves; however, and there are some downsides to using black-box explainers. The explanations from these models assist in visualization, but they result in an explanation of a black-box that was generated by a black-box. With this in mind, how can the explanation generated by the black box explainer be trusted if there is no way to visualize \textbf{or verify} the method that was used to create the explanation? The alternative to black-box explanation is \textcolor{red}{white-box explanation}. \textcolor{red}{In this work,} we have chosen \textcolor{red}{white-box} rule extraction as it is a strong counterpart to black-box explainability. Rule extraction algorithms construct a trustworthy model that is composed of ANN decisions that are expressed as sets of rules.

Rule Extraction (RE) is the process of generating rules by using the black-box ANN's input, hidden, and output layers. RE can refer to three different techniques: decompositional, pedegogical, and eclectic \cite{hailesilassie2016rule}. The decompositional approach decomposes the neural network from output to input, iteratively generating rules that connect the input and output layers. Pedagogical algorithms focus solely on generating rules using the ANN's inputs and outputs. This technique ignores the hidden layer weights all together. Lastly, eclectic algorithms use ideas from both the previous techniques. This technique does not decompose the entire network, rather it uses the hidden layers in combination with model outputs to generate rules. Due to this, eclectic algorithms are able to be flexible in how they are trained and are a prime candidate for Deep Neural Network (DNN) X-IDS.


In this paper, we present an eclectic rule extraction algorithm that explains a DNN IDS. The proposed solution is a white-box surrogate explainer that utilizes the DNN's hidden layers to generate an explainable ruleset. DNN models are created using the UNSW-NB15 and CIC-IDS-2017 datasets, and explainable rulesets are created using the eclectic RE algorithm. We find that the RE algorithm is able to generate rulesets that mimic the models' outputs at an accuracy of 99.9\%. Additionally, the rulesets have similar accuracy of within 1\% to the DNN models when compared to the datasets' ground truth labels.


%In \cite{aytekin2022neural} the author showed that, ANNs can be converted to decision trees and explained. Additionally, \cite{frosst2017distilling} is similar to the previous work, albeit with a more detailed approach to convert an ANN to a decision tree. ANN to decision tree conversion is relatively simple, considering a neuron firing is binary, especially in ANNs using ReLU as the activation function. The decision tree approach eliminates the shortcomings of the black box approaches, as decision trees are opaque models. Explanation of a black box model with a white box explainer provides a certain degree of explainability that other approaches cannot. Additionally the decision tree conversion model provides both local and global explanations which results in a broader overview of the results.


Major contributions presented in this paper are -
\begin{itemize}
    \item A hybrid X-IDS architecture using a black box DNN predictor and a white box surrogate explainer. Eclectic RE is used to generate human-readable rules from the hidden nodes of a DNN. RE creates a global, explainable ruleset that can be used to help users understand how and why their model makes predictions.

    \item An eclectic rule extraction algorithm that can be run on intrusion detection datasets. This algorithm can be run for both binary and categorical predictions. An eclectic RE algorithm gives the user flexibility when determining how much of the model they would like to explain. This can greatly increase the explanation creation's performance. This RE algorithm is able to create high-accuracy rulesets.
    
    \item A performative and explanatory analysis of our architecture using modern datasets. Our model is tested against the CIC-IDS-2017 and UNSW-NB15 datasets. Using these datasets, we train and test our DNN and create accurate rulesets. Rulesets are able to mimic the DNNs' outputs with an accuracy of 99.9\%. We discuss the trade-off of speed and performance and detail the rulesets' explainablity. %It is able to achieve an accuracy of 99.6\% on CIC-IDS-2017 and \hl{97\%} on UNSW-NB15. 
    
\end{itemize}

==> old_section3.tex <==
\section{Surrogate Explainers}
\label{sec: surrogate explainers}

A popular category of explainer algorithms in IDS applications is surrogate explainers. This section analyses a few of the popular surrogate explainers, their applications in IDSs, a comparison of their performance, and the reasoning behind our decision to utilize rule extraction. Just like classifiers, surrogate explainers may have either a black box or white box architecture. Black box explainers like LIME \cite{Ribeiro2016}, SHAP \cite{Lundberg2017}, and LRP are cutting edge surrogate explainers, and they are often used to explain the decisions of IDS systems \hl{add a couple citations here of works that used them}. However, there are some white box surrogate explainers as well, such as, Bayesian Rule Lists \cite{yang2017scalable}, or in the case of this paper, DTA \hl{we have moved to calling it rule extraction. similar but different in a way} \cite{aytekin2022neural, blanco2019machine}

\subsection{Black Box Explainers}
\textcolor{red}{Black Box surrogate explainers typically All of the black box explainers mentioned here LIME takes in a specific sample, then it formulates its explanations by creating perturbations of that sample and training a surrogate model on the perturbations.} \hl{imma need u to reread this sentence} SHAP makes its predictions by choosing a neutral point, examining all permutations of the data, specifically individual combinations of features. The model then calculates the Shapley values for each feature, and combinations of the features. The calculation of the Shapley values provides each feature's contribution to the model's decision. The last black box surrogate explainer considered in this work is LRP. \hl{NOTE: Add information about LRP | FIND CORRECT CITATION}

\subsection{White Box Explainers}
A strong white box explainer and the focus of this paper is decision tree analysis. Essentially, in DTA, a surrogate model (decision tree) is generated based on a set of predetermined criteria. In DTA a binary tree is generated where each leaf is one of the ANN's decisions, this allows the individual decisions of the ANN to be easily visualized. Considering the opaqueness of the decision tree's structure, both global and local explainability are built in. \cite{blanco2019machine}  \hl{NOTE: Examine the source}
\hl{NOTE: Add additional information about WB surrogates}

\subsection{Performance Analysis}
Despite their success, the black box models discussed here are not without flaws. For example, LIME and SHAP may not provide global explanations within their base implementations. Additionally, Shapley values are computationally expensive, this becomes more noticeable on datasets with many of features. Lastly, black box surrogate explainers can be difficult to verify. This may lead to concerns surrounding the validity of the explanations themselves. DTA tends to be more robust than it's black box counterparts, as any ANN can be converted into a decision tree \cite{aytekin2022neural, frosst2017distilling}. However, a notable problem with DTA is that the size of the tree is directly proportional to the size of the ANN.

The previously stated issues do not encompass the inspiration for this work, however. A deep neural network can be visualized as the simplified mathematical structure: $$ f(x): x \rightarrow y, x \in X, y \in Y $$ where x is a sample from the dataset X, and y is a prediction that falls within the collection of valid outputs Y. The lack of explainability in black box models is derived from the fact that the inner workings of the model cannot be observed. 

In this paper, we take on the perspective that, black box explainers inevitably circle back to the same problems that black box classifiers possess. For example, when explaining a black box ANN with a black box explainer, the same problem is encountered at both phases of the explanation. Explainers are applied to models to determine their validity, but if the explainers in question are also black boxes, how can the explainers' accuracy and reliability be determined? \hl{Probably needs rewording} This is why the focus of this paper is explainability using a decision tree surrogate explainer. As stated in \cite{frosst2017distilling} an ANN can be converted to a decision tree with relative ease and with little change to the accuracy of the model, as seen in Section \hl{Insert section} \hl{STOP}
